Monocular Depth Parameterizing Networks

Monocular depth estimation is a highly challenging problem that is often addressed with deep neural networks. While these are able to use recognition of image features to predict reasonably looking depth maps the result often has low metric accuracy. In contrast traditional stereo methods using multiple cameras provide highly accurate estimation when pixel matching is possible. In this work we propose to combine the two approaches leveraging their respective strengths. For this purpose we propose a network structure that given an image provides a parameterization of a set of depth maps with feasible shapes. Optimizing over the parameterization then allows us to search the shapes for a photo consistent solution with respect to other images. This allows us to enforce geometric properties that are difficult to observe in single image as well as relaxes the learning problem allowing us to use relatively small networks. Our experimental evaluation shows that our method generates more accurate depth maps and generalizes better than competing state-of-the-art approaches.

==> Generate_illustrations/idasfigur.tex <==
\begin{tikzpicture}[xscale=0.25, yscale=0.25]
% (Default height of block is h = 12)

%\node[inner sep=0pt] (439_stress) at (1.55,7.45)
%    {\includegraphics[width=7.7mm]{439_stress.jpg}};
\node[yslant=-1.,inner sep=0pt] (439_stress) at (1.55,7.45)
    {\includegraphics[width=7.7mm, height=22.3mm]{Images/Doge_Palace_R5.png}};%{439_stress.jpg}};
%\node[xslant=0.5, draw] at ([yshift=10]1.north) {\includegraphics[width=7.7mm]{439_stress.jpg}}

\edef\x{0}
\edef\h{12}
\def\o{1.5+6-\h*0.5}
\def\b{3*\h/12}
\foreach \w/\imSize/\ch/\op in {0.15/296/2/C3+M, 1.5/147/4/C4+M, 1.5/72/4/C3+M, 2.8/35/8/C4+M, 2.8/16/8/C3+M, 5.4/7/16/C4, 5.4/4/16/C4}{
    % Block
    \filldraw[fill=gray!90] 
        (\x+\b,\o) -- (\x+\b+\w,\o) -- (\x+\b+\w,\o+\h-\b) -- (\x+\b,\o+\h-\b);
    \filldraw[fill=gray!90] 
        (\x+\b,\o+\h-\b) -- (\x+\b+\w,\o+\h-\b) -- (\x+\w,\o+\h) -- (\x,\o+\h);
    \draw (\x+\b,\o) -- (\x,\o+\b) -- (\x,\o+\h) -- (\x+\b,\o+\h-\b) -- (\x+\b,\o) -- (\x+\b+\w,\o) -- (\x+\b+\w,\o+\h-\b) -- (\x+\b,\o+\h-\b) -- (\x+\b+\w,\o+\h-\b) -- (\x+\w,\o+\h) -- (\x,\o+\h);
    
    %Text
    \node[draw=none] at (\x-.3,\o+\b*.7-.8) {\scriptsize{\imSize}};
    \node[draw=none] at (\x+\b+\w/2,\o-1.2) {\scriptsize{\ch}};
    \node[draw=none] at (\x+\b+\w*1.2,\o+\h+1.3) {\footnotesize{\op}};
    
    % Update parameters
    \pgfmathparse{\x+\w+\b+1.8}
    \xdef\x{\pgfmathresult}
    \pgfmathparse{\h*0.65}
    \xdef\h{\pgfmathresult}
    \xdef\o{1.5+6-\h*0.5}
    \xdef\b{3*\h/12}
    }

\xdef\s{1}
\xdef\d{.6}
% First flat layer
\foreach \i in {1,2,...,4}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
\pgfmathparse{\x+\d/2}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2,3}
    \pgfmathparse{\x+.3}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=.01,draw,fill=black](circ1) at (\x,7.5){};
\foreach \i in {1,2,...,4}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
% Text
\node[draw=none] at (\x-4*\d-.3,\o-1.2) {\scriptsize{32}};


% Additional data layer
\pgfmathparse{\x+.3}
\xdef\x{\pgfmathresult}
\node[draw=none] at (\x+0.7,7.5) {\footnotesize{+}};


\pgfmathparse{\x+1}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2,...,6}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
\pgfmathparse{\x+1}
\xdef\x{\pgfmathresult}
% Text
\node[draw=none] at (\x-2*\d-1.4,\o-1.2) {\scriptsize{BMI}};%\x-2*\d-1.2
\node[draw=none] at (\x-2*\d-1.4,\o-2.5) {\scriptsize{Age}};
\node[draw=none] at (\x-2*\d-1.4,\o-3.8) {\scriptsize{Sex}};
\node[draw=none] at (\x-2*\d-1.4,\o-5.1) {\scriptsize{Angina symp.}};
\node[draw=none] at (\x-2*\d-1.4,\o-6.4) {\scriptsize{Pre-test prob.}};
\node[draw=none] at (\x-2*\d-1.4,\o-7.7) {\scriptsize{AHA}};
%\node[draw=none] at (\x-2*\d-1.2,\o-1.2) {\scriptsize{BMI, Age}};
%\node[draw=none] at (\x-2*\d-1.2,\o-2.5) {\scriptsize{Sex, Angina}};
%\node[draw=none] at (\x-2*\d-1.2,\o-3.8) {\scriptsize{Pre-test prob., AHA}};
%\node[draw=none] at (\x-2*\d-.3,\o-1.2) {\scriptsize{-}};
\pgfmathparse{\x+.3}
\xdef\x{\pgfmathresult}
\node[draw=none] at (\x,1.5+6-\h*0.5/0.65+\h/0.65+1.3) {\footnotesize{C1}};
\pgfmathparse{\x+1}
\xdef\x{\pgfmathresult}

\draw[densely dashed] (\x-6.8,\o+1.2) -- (\x-6.8,\o-8.5) -- (\x-.9,\o-8.5) -- (\x-.9,\o+1.2) -- (\x-6.8,\o+1.2);

% Second flat layer
\foreach \i in {1,2}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
\pgfmathparse{\x+\d/2}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2,3}
    \pgfmathparse{\x+.3}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=.01,draw,fill=black](circ1) at (\x,7.5){};
\foreach \i in {1,2}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
% Text
\node[draw=none] at (\x-2*\d-.3,\o-1.2) {\scriptsize{32}};
\node[draw=none] at (\x+1.3,1.5+6-\h*0.5/0.65+\h/0.65+1.3) {\footnotesize{C1}};

% Third flat layer
\pgfmathparse{\x+2}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
\pgfmathparse{\x+\d/2}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2,3}
    \pgfmathparse{\x+.3}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=.01,draw,fill=black](circ1) at (\x,7.5){};
\foreach \i in {1,2}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
% Text
\node[draw=none] at (\x-2*\d-.3,\o-1.2) {\scriptsize{16}};
\node[draw=none] at (\x+1.3,1.5+6-\h*0.5/0.65+\h/0.65+1.3) {\footnotesize{C1}};
    
% Fourth flat layer
\pgfmathparse{\x+2}
\xdef\x{\pgfmathresult}
\foreach \i in {1,2,...,3}
    \pgfmathparse{\x+\d}
    \xdef\x{\pgfmathresult}
	\node[circle,inner sep=\s,draw,fill=gray!90](circ1) at (\x,7.5){};
% Text
\node[draw=none] at (\x-\d*1,\o-1.2) {\scriptsize{3}};

% To make figure not end too far to the right
\node[draw=none] at (\x+\d,\o) {\scriptsize{}};

%\draw [thick,decoration={brace, mirror, raise=5pt}, decorate] (\x-\d*1.5-2,5.5) -- node[below=10pt] {Class label \textit{y}} (\x-\d*1.5+2,5.5); 

\end{tikzpicture}

==> Images/FiguresAblation.tex <==
\begin{figure*}[ht!]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics[width = 18mm]{Images/MonoVsPhotometric/image/1311867723.009268_rgb.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/gt/1311867723.009268_.png}
        \includegraphics[width = 18mm]{Images/MonoVsPhotometric/image/1311867818.331196_rgb.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/gt/1311867818.331196_.png}
        \includegraphics[width = 18mm]{Images/MonoVsPhotometric/image/1311867723.009268_rgb.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/gt/1311867723.009268_.png} \hspace{0.3cm}   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/image/1311867723.009268_rgb.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/gt/1311867723.009268_.png}  \includegraphics[width = 18mm]{Images/MonoVsPhotometric/image/1311867723.009268_rgb.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/gt/1311867723.009268_.png}
   \vspace{0.3cm}  \includegraphics[width = 18mm]{Images/MonoVsPhotometric/0739gt.png}
   }\\\resizebox{\textwidth}{!}{
    \includegraphics[width = 18mm]{Images/MonoVsPhotometric/monocular/1311867723.009268_.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/photometric/1311867723.009268_.png}
      \includegraphics[width = 18mm]{Images/MonoVsPhotometric/monocular/1311867818.331196_.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/photometric/1311867818.331196_.png}
    \includegraphics[width = 18mm]{Images/MonoVsPhotometric/monocular/1311867723.009268_.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/photometric/1311867723.009268_.png} \hspace{0.3cm}
     \includegraphics[width = 18mm]{Images/MonoVsPhotometric/monocular/1311867723.009268_.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/photometric/1311867723.009268_.png}
    \includegraphics[width = 18mm]{Images/MonoVsPhotometric/monocular/1311867723.009268_.png}
   \includegraphics[width = 18mm]{Images/MonoVsPhotometric/photometric/1311867723.009268_.png} \includegraphics[width = 18mm]{Images/MonoVsPhotometric/0739gt.png}
   }\\ \resizebox{\textwidth}{!}{\includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
    \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \hspace{0.3cm}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}
   \includegraphics[width = 18mm]{Images/eglise/DSC_0007.JPG}\vspace{0.3cm}  \includegraphics[width = 18mm]{Images/MonoVsPhotometric/0739gt.png}}
   \vspace{-0.5cm}
    \label{fig:my_label}
    \caption{\textbf{Ablation studies}. }
\end{figure*}

==> Images/Stereosmall.tex <==
\begin{figure}
 \begin{subfigure}[b]{0.24\textwidth} 
 \centering
 \vspace{0.3cm}
  \includegraphics[width = 1.3cm]{Images/Stereoimages/image/frame-000377.jpg}
     \includegraphics[width = 1.3cm]{Images/Stereoimages/1rgb.png}
      \includegraphics[width = 1.3cm]{Images/Stereoimages/2rgb.png}
\\
       \vspace{-0.45cm}
       \resizebox{\textwidth}{!}{\hspace{0.1cm}\tiny{\alert{\textbf{scannet/scene0799\_00}}}\hspace{0.5cm}
       \alert{\textbf{TUM/seq3}}\hspace{1.3cm}
       \alert{\textbf{TUM/seq3}}\hspace{1.2cm}}
       \\
        \includegraphics[width = 1.3cm]{Images/Stereoimages/gt/frame-000377.jpg_.png}
        \includegraphics[width = 1.3cm]{Images/Stereoimages/1gt.png}
      \includegraphics[width = 1.3cm]{Images/Stereoimages/2gt.png}
      \\ 
        \includegraphics[width = 1.3cm]{Images/Stereoimages/stereo/stereo_frame-000377.png}
        \includegraphics[width = 1.3cm]{Images/Stereoimages/1img1Disp_matl.png}
      \includegraphics[width = 1.3cm]{Images/Stereoimages/2img1Disp_matl.png}
\\ 
\includegraphics[width = 1.3cm]{Images/Stereoimages/photo/frame-000377.jpg_.png}
       \includegraphics[width = 1.3cm]{Images/Stereoimages/1our.png}
      \includegraphics[width = 1.3cm]{Images/Stereoimages/2our.png}
      \\
     \end{subfigure}\hspace{0.5cm}
     \begin{subfigure}[b]{0.2\textwidth}
 \resizebox{0.55\textwidth}{!}{
     \includegraphics[width = 2.3cm, trim = 150 180 150 0]{Images/MonoVsPhotometric/0799_00_frame-000372_mono00.png}}
     \tiny{\textbf{Stereo}}\\
     \resizebox{0.55\textwidth}{!}{ \includegraphics[width = 2.3cm, trim = 150 150 150 150]{Images/MonoVsPhotometric/0799_00_frame-000372_our01.png}}\hspace{0.2cm}\tiny{\textbf{Photometric}}\\
       \end{subfigure}
       \caption{Comparison of depth maps produced by stereo method and ours. The left images correspond to input image , ground truth, stereo depth and Photometric (ours) (from upper to lower). The right images shows reconstruction from scannet scene0799\_00 for stereo and Photometric depth. }
    %\label{fig:my_label}
\end{figure}

==> Images/frontpage_other.tex <==
\begin{figure}[ht!]
    \centering
\resizebox{0.4\textwidth}{!}{\includegraphics[ width = 6cm]{Images/Comparing_all/images/frame-000730.jpg}\hspace{3cm}
\includegraphics[ width = 4cm,trim = 200 200 250 220]{Images/3D_comp_all/Ours/frame-00073400.png}\hspace{3cm}}\\
 \resizebox{0.4\textwidth}{!}{\vspace{-6cm}\hspace{3cm}\footnotesize{\textbf{Image}}\hspace{4cm}\footnotesize{\textbf{Ours}}\hspace{0cm}}
\resizebox{0.4\textwidth}{!}{
\includegraphics[ width = 3cm,trim = 90 90 90 190]{Images/3D_comp_all/DF/frame-00073401.png}
\includegraphics[ width = 3cm,trim = 90 190 90 120]{Images/3D_comp_all/MD/frame-00073401.png}
}
\\
\vspace{-0.7cm}
 \resizebox{0.45\textwidth}{!}{\vspace{-6cm}\hspace{4cm}\footnotesize{\textbf{Deepfactors}}\hspace{3cm}\footnotesize{\textbf{Megadepth}}}
\vspace{0.5cm}
    \caption{Our monocular depth parameterizing network produces high quality and detailed reconstructions. We achieve realistic looking depth maps and reconstructions for a large variety of scenes.  }
    \label{fig:bad_momodepth}
\end{figure}

\begin{figure}[ht!]
    \centering
    \hspace{-1cm}
  \resizebox{0.4\textwidth}{!}{   \includegraphics[width = 18mm]{Images/Comparing_all/images/1341847989.402777_rgb.png}
 \includegraphics[width = 22mm, trim = 80 210 100 100]{Images/Comparing_all/ours/1341847989.40277701.png}}
 \resizebox{0.4\textwidth}{!}{\vspace{-6cm}\hspace{3cm}\footnotesize{\textbf{Image}}\hspace{3cm}\footnotesize{\textbf{Ours}}\hspace{1cm}}
 \resizebox{0.4\textwidth}{!}{   \includegraphics[width = 18mm, trim = 100 80 80 140]{Images/Comparing_all/Deepfactors/1341847989.40277701.png}\includegraphics[width = 18mm, trim = 60 100 100 100]{Images/Comparing_all/megadepth/1341847989.40277701.png}
}
\\
\vspace{-0.5cm}
\hspace{-0.5cm}
 \resizebox{0.48\textwidth}{!}{\vspace{-6cm}\hspace{4cm}\footnotesize{\textbf{DeepFactors \cite{Czarnowski:2020:10.1109/lra.2020.2965415}}}\hspace{3cm}\footnotesize{\textbf{MegaDepth \cite{li2018megadepth}}}}
    \caption{Our monocular depth parameterizing network produces high quality and detailed reconstructions. We achieve realistic-looking depth maps and reconstructions for a large variety of scenes.  }
    \label{fig:bad_momodepth}
\end{figure}

\begin{figure}[ht!]
    \centering
  \resizebox{0.4\textwidth}{!}{   \includegraphics[width = 18mm]{Images/Comparing_all/images/1341839268.304930_rgb.png}    
 \includegraphics[width = 22mm, trim = 20 180 80 80]{Images/3D_comp_all/Ours/1341839269.84482800.png}
 }
 \resizebox{0.4\textwidth}{!}{\vspace{-6cm}\hspace{3cm}\footnotesize{\textbf{Image}}\hspace{3cm}\footnotesize{\textbf{Ours}}\hspace{1cm}}
 \resizebox{0.4\textwidth}{!}{   \includegraphics[width = 18mm, trim = 100 80 80 140]{Images/3D_comp_all/DF/1341839269.84482800.png}\includegraphics[width = 18mm, trim = 60 100 100 100]{Images/3D_comp_all/MD/1341839269.84482800.png}
}
\\
\vspace{-0.8cm}
 \resizebox{0.45\textwidth}{!}{\vspace{-6cm}\hspace{4cm}\footnotesize{\textbf{DeepFactors \cite{Czarnowski:2020:10.1109/lra.2020.2965415}}}\hspace{3cm}\footnotesize{\textbf{MegaDepth \cite{li2018megadepth}}}}
    \caption{Our monocular depth parameterizing network produces high quality and detailed reconstructions. We achieve realistic-looking depth maps and reconstructions for a large variety of scenes.  }
    \label{fig:bad_momodepth}
\end{figure}

==> tables/tableablation_mono.tex <==
\begin{table}[!htbp]
\begin{center}
\resizebox{0.48\textwidth}{!}{\begin{tabular}[ht!]{|l|l|c c|c c|}
\hline
 & & \multicolumn{2}{|c|}{lower is better} & \multicolumn{2}{|c|}{higher is better}\\
Dataset & Method
&Abs Rel  &RMSE log & $\delta<1.1$ & $\delta<1.25$  \\ %\midrule
\hline
\textbf{Scannet/scene0707\_00}&Monodepth & 0.1590 & 0.0182& 39.79\% & 77.14\%\\ 
&Photometric & 0.0805 & 0.0071& 73.50\% & 93.44\%\\ 
\hline
\textbf{Scannet/scene0715\_00}&Monodepth & 0.1097& 0.0100 & 56.27\% & 88.46\%\\ 
&Photometric & 0.0582 & 0.0045& 83.40\%&  96.67\%\\  \hline

\textbf{Scannet/scene0799\_00}&Monodepth & 0.1568& 0.0197 & 46.30\% & 76.33\%  \\
&Photometric &0.0658 & 0.0056  & 79.43\% & 95.00\%  \\
\hline
\textbf{TUM/seq1}&Monodepth & 0.1710& 0.2136& 35.86\% &70.61\% \\ 
&Photometric & 0.1261 & 0.0164& 72.43\% & 83.56\% \\
\hline
\textbf{TUM/seq2}&Monodepth & 0.5670& 0.0256 & 32.76\% & 77.14\% \\ 
&Photometric & 0.0409& 0.0063& 90.56\% & 95.57\%\\
\hline
\textbf{TUM/seq3} &Monodepth &0.2005 & 0.0491 &  38.57\% & 68.08\%\\ 
&Photometric &0.0910 &0.0187 & 74.93\% & 88.25\%\\
\hline
\end{tabular}}
\caption{\textbf{Ablation study.} Metrics comparing ours (Photometric) with Monocular depth estimation, considering test datasets scannet \cite{dai2017scannet} and TUM \cite{sturm12iros}. The networks are both solely trained supervised on the scannet training datasets. All presented metrics are presented as mean over number of samples. \alert{Updated and done}}
\label{table:monovsphotometric}
\end{center}
\end{table}


==> tables/tableablation_stereo.tex <==
\begin{table}[!htbp]
\begin{center}
\resizebox{0.48\textwidth}{!}{\begin{tabular}[h]{|l|l|c c|c c|}
\hline
 & & \multicolumn{2}{|c|}{lower is better} & \multicolumn{2}{|c|}{higher is better}\\
Dataset & Method
&absrel  &log RMSE$^{sc.}_{inv.}$ & $\delta<1.1$ & $\delta<1.25$ \\ %\midrule
\hline\hline
\textbf{Scannet/scene0707\_00}&Stereo  &  0.1330  & 0.2119 & 58.02\% & 84.79\% \\ 
&Photometric (Ours) & 0.1384 & 0.0186& 57.39\% & 82.80\%\\ 
\hline
\textbf{Scannet/scene0715\_00}&Stereo & 0.1609 & 2.2170 &  55.87\% &  78.94\% \\
&Photometric (Ours) & 0.1157 &  0.0171  & 63.75\% & 85.08\% \\
\hline
\textbf{Scannet/scene0799\_00}& Stereo& 0.1866&0.9313 &  50.48\%& 74.13\%\\ 
&Photometric (Ours)&0.1125& 0.0164& 64.48\% & 85.33\% \\
\hline
\textbf{TUM/seq1}& Stereo& 0.2832& 8.4654& 65.15\% & 76.58\% \\ 
&Photometric (Ours)& 0.1492 & 0.0212& 67.75\% & 80.20\% \\
\hline
\textbf{TUM/seq2}& Stereo & 0.1350& 7.1718& 57.82\% &  80.18\%\\ 
&Photometric (Ours)& 0.0588& 0.0095& 87.40\% & 93.43\%\\
\hline
\textbf{TUM/seq3}& Stereo & 0.1350& 7.1718& 57.82\% & 80.18\%\\ 
&Photometric (Ours) & 0.1134& 0.0282& 67.97\% &  85.25\%\\
\hline
\end{tabular}} 
\caption{Results comparing ours Photometric with 2 covisible cameras with Stereo method in \cite{olsson-etal-cvpr-2013}. The considering datasets scannet \cite{dai2017scannet} and TUM \cite{sturm12iros}. All presented metrics are presented as mean over number of samples. \alert{Updated and done}}
\label{table:stereo}
\end{center}
\end{table}


==> tables/tables_old.tex <==
\begin{table*}[ht!]
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{|l|l|c c c c|c c c|}
\hline
 & & \multicolumn{4}{|c|}{lower is better} & \multicolumn{3}{|c|}{higher is better}\\
Dataset/scene & Method
&Abs Rel & Sq Rel  & RMSE &RMSE log & pc110 & $\delta < 1.25$& $\delta < 1.25^2$\\ %\midrule
\hline\hline
\textbf{scannet/scene0565\_00}&Deepfactors & 0.1494 &&&0.0198& 47.16\%& 77.10\%& 95.76\%\\ 
&MegaDepth &  &&& & & & \\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours  & \textbf{0.0980}&&& \textbf{0.0106} & \textbf{67.31\%} & \textbf{88.70\%}&\textbf{97.83\%} \\ 
\hline
\textbf{scannet/scene0606\_02}&Deepfactors & 0.1736 &&&0.455 &44.52\%&73.09\% & 91.01\% \\ 
&MegaDepth &  & & & & & & \\ 
&PSMNet &  & & & & & & \\ 
%&Deep stereo  & & &\\ 
&Ours  & \textbf{0.1232}&& & \textbf{0.0192} &  \textbf{61.43\%}& \textbf{83.75\%}& \textbf{95.45\%}\\  \hline
\textbf{scannet/scene0715\_00}&Deepfactors & 0.0926& &&0.0098 &64.90\%&91.23\% & 98.21\%\\ 
&MegaDepth  & &&& & & & \\ 
&PSMNet & 0.1609 & 0.4437& 0.8163 & 2.217& 55.87\% & 78.93\%& 90.45\% \\ 
%&Deep stereo  & & &\\ 
&Ours  & \textbf{0.0674}& &&\textbf{0.0065}& \textbf{79.42\%}&\textbf{94.69\% }& \textbf{98.68\%}\\ 
\hline
\textbf{scannet/scene0743\_00}&Deepfactors & 0.1532&&& 0.2493& 46.15\%&78.43\% & 95.69\%\\  
&MegaDepth  &&& & && & \\  
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours  & \textbf{0.0819} &&& \textbf{0.0073} & \textbf{72.01\%}& \textbf{92.60\%}& \textbf{98.68\%}\\  \hline
\textbf{scannet/scene0799\_00}& Deepfactors & 0.1523& &&0.0219& 50.27\%&76.22\% & 94.64\%\\ 
&MegaDepth & &&& && & \\  
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours  & \textbf{0.0808} &&& \textbf{0.0088 }& \textbf{73.52\%}&\textbf{91.35\%} & \textbf{98.02\%}\\ \hline
\textbf{TUM/freiburg2\_rpy}& Deepfactors & \textbf{0.2282} & &&4.9252& \textbf{43.9253\%}& \textbf{68.69\%}& \textbf{82.97\%}\\ 
&MegaDepth  & & && & \\  
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours & 0.249 &&& \textbf{4.623}& 37.26\%&62.49\% &76.41\% \\  \hline
\textbf{TUM/freiburg3\_structure\_texture\_far\_validation}&Deepfactors & 0.1259&&& 0.0186&53.26\%& 83.59\% &95.34\% \\
&MegaDepth  & &&& && & \\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours & \textbf{0.068} &&&\textbf{0.0134} & \textbf{85.37\%}& \textbf{91.38\%}& \textbf{96.52\%} \\ \hline
\textbf{TUM/freiburg3\_structure\_texture\_far}&Deepfactors & 0.1102 &&&0.0143 & 57.85\%&86.65\% &96.30\% \\ 
&MegaDepth  &&& & && & \\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours & \textbf{0.047} &&& \textbf{0.0075} &  \textbf{91.44\%}& \textbf{95.74\%}& \textbf{97.82\%}\\  \hline
\textbf{TUM/freiburg3\_nostructure\_texture\_near\_withloop}&Deepfactors & \textbf{0.1516} &&& 1.0614 & 41.8756\%&\textbf{77.44\%} & \textbf{97.41\%}\\  
&MegaDepth  & &&& && &\\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
& Ours & 0.20457 &&& \textbf{0.0334} &\textbf{ 59.18\%}&73.32\% &87.66\% \\  \hline
\textbf{TUM/freiburg3\_long\_office\_household} & Deepfactors & 0.1751 &&& 0.0486& 45.89\%& 74.56\%& 88.21\%\\ 
&MegaDepth &  &&& & & & \\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours & \textbf{0.1273} & &&\textbf{0.0359 }& \textbf{64.09\%}& \textbf{82.20\%}& \textbf{90.47\%}\\  \hline
\textbf{TUM/freiburg1\_xyz} & Deepfactors &0.1154 &&&0.265 &  58.42\%& 85.87\%& 95.81\%\\ 
&MegaDepth  &&& & && & \\ 
&PSMNet &  &&& & & & \\ 
%&Deep stereo  & & &\\ 
&Ours &\textbf{ 0.0965}&&& \textbf{0.014}& \textbf{69.03\%}& \textbf{87.32\%}&\textbf{96.15\%} \\  \hline
\end{tabular}}
\caption{\textbf{Quantitative results.} Comparison of existing methods to our own on Scannet scenes [] and TUM RBG-D[]. }
\end{center}
\end{table*}

==> tables/tabletrainingold.tex <==
\begin{table}[!htbp]
\begin{center}
\resizebox{0.48\textwidth}{!}{\begin{tabular}[h]{|l|l|c c|c c|}
\hline
 & & \multicolumn{2}{|c|}{lower is better} & \multicolumn{2}{|c|}{higher is better}\\
Dataset & Method
&absrel  &log RMSE$^{sc.}_{inv.}$& $\delta<1.1$ & $\delta<1.25$ \\ %\midrule
\hline\hline
\textbf{scannet/scene0707\_00}&Supervised & 0.0805 & 0.0071  &73.50\%& 93.44\% \\ 
&Self-supervised & 0.0916 &  0.0091 & 68.65\% & 91.10\%\\ 
\hline
\textbf{scannet/scene0715\_00}&Supervised & 0.0582&0.0045& 83.40\% & 96.67\% \\
&Self-supervised & 0.0672  & 0.0065 & 79.63\% & 94.75\% \\
\hline
\textbf{scannet/scene0799\_00}&Supervised & 0.0658& 0.0056& 79.43\% & 95.00\%\\ 
&Self-supervised & 0.0805& 0.0088& 73.64\%& 91.41\% \\
\hline
\textbf{TUM/seq1}&Supervised &  0.1261 & 0.0164& 72.43\% & 83.56\% \\
&Self-supervised& 0.1871 & 0.0286&65.82\% & 74.56\% \\
\hline
\textbf{TUM/seq2}&Supervised & 0.0409& 0.0063& 90.56\% & 95.57\% \\ 
&Self-supervised& 0.0497& 0.0084& 88.49\% & 92.83\%\\
\hline
\textbf{TUM/seq3} &Supervised & 0.0910 & 0.0187& 74.93\% & 88.25\%\\ 
&Self-supervised & 0.1030& 0.0248& 71.89\% & 86.06\%\\
\hline
\end{tabular}} 
\caption{Evaluation of training approach, comparing networks that have been trained supervised and weakly supervised. }
\label{table:traing}
\end{center}
\end{table}

